Recognize Any Regions

Understanding the semantics of individual regions or patches of unconstrained images, such as open-world object detection, remains a critical yet challenging task in computer vision. Building on the success of powerful image-level vision-language (ViL) foundation models like CLIP, recent efforts have sought to harness their capabilities by either training a contrastive model from scratch with an extensive collection of region-label pairs or aligning the outputs of a detection model with image-level representations of region proposals. Despite notable progress, these approaches are plagued by computationally intensive training requirements, susceptibility to data noise, and deficiency in contextual information. To address these limitations, we explore the synergistic potential of off-the-shelf foundation models, leveraging their respective strengths in localization and semantics. We introduce a novel, generic, and efficient architecture, named RegionSpot, designed to integrate position-aware localization knowledge from a localization foundation model (e.g., SAM) with semantic information from a ViL model (e.g., CLIP). To fully exploit pretrained knowledge while minimizing training overhead, we keep both foundation models frozen, focusing optimization efforts solely on a lightweight attention-based knowledge integration module. Extensive experiments in open-world object recognition show that our RegionSpot achieves significant performance gain over prior alternatives, along with substantial computational savings (e.g., training our model with 3 million data in a single day using 8 V100 GPUs). RegionSpot outperforms GLIP-L by 2.9 in mAP on LVIS val set, with an even larger margin of 13.1 AP for more challenging and rare categories, and a 2.5 AP increase on ODinW. Furthermore, it exceeds GroundingDINO-L by 11.0 AP for rare categories on the LVIS minival set.

==> table/abl_sam.tex <==
\begin{table}[tb]\centering
    \caption{Results of training on ADE20K panoptic and evaluating on COCO panoptic val set}
    \label{tab:ade_train}
    \resizebox{0.5\textwidth}{!}{
    \large
    \begin{tabular}{c|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c}{ADE20K} \\
       Method & PQ & SQ & RQ & PQ & SQ & RQ \\
        \midrule
        ODISE & 25.0 & 79.4  & 30.4& 31.4 & 77.9 & 36.9\\
        FC-CLIP & 27.0 &78.0 &32.9 &41.9 &78.2 &50.2\\
        Ours &  &   &   &   &   & \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> table/ade_train.tex <==
\begin{table}[tb]\centering
    \caption{Results of training on ADE20K panoptic and evaluating on COCO panoptic val set}
    \label{tab:ade_train}
    \resizebox{0.5\textwidth}{!}{
    \large
    \begin{tabular}{c|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{COCO} & \multicolumn{3}{c}{ADE20K} \\
       Method & PQ & SQ & RQ & PQ & SQ & RQ \\
        \midrule
        ODISE & 25.0 & 79.4  & 30.4& 31.4 & 77.9 & 36.9\\
        FC-CLIP & 27.0 &78.0 &32.9 &41.9 &78.2 &50.2\\
        Ours &  &   &   &   &   & \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> table/main_table.tex <==
\begin{table}[t]
\centering
\caption{Comparison of open-world zero-shot object recognition performance using ground-truth (GT) boxes, RPN boxes, and GLIP boxes on the LVIS dataset.}
% \footnotesize
\begin{tabular}{l|c|c|c|c|c|c}
Method & Training Data & Proposals & Params & AP$_{r}$ & AP$_{f}$ & AP$_{all}$ \\
\shline \hline
CLIP w/ box & - & GT & - & 40.6 & 59.2 & 48.7 \\
CLIP w/ mask & - & GT & - & 40.8 & 59.6 & 49.2 \\
RegionCLIP & CC3M & GT & 87 & 50.1 & 51.7 & 50.7 \\
\rowcolor{cyan!50}
\modelnamelite & O365, OI, V3D & GT & 22 & 42.0 & 65.6 & 53.0 \\
\rowcolor{cyan!50}
\modelnamepro & O365, OI, V3D & GT & 35 & {50.6} & {68.8} & {56.6} \\
\rowcolor{cyan!50}
\modelnameproplus & O365, OI, V3D & GT & 35 & \textbf{55.4} & \textbf{68.6} & \textbf{59.9} \\
\hline
RegionCLIP & CC3M & RPN & 87 & 13.8 & 9.4 & 11.3 \\
\rowcolor{cyan!50}
\modelnamelite & O365, OI, V3D & RPN & 22 & 10.9 & 13.6 & 11.8 \\
\rowcolor{cyan!50}
\modelnamepro & O365, OI, V3D & RPN & 35 & 12.7 & {15.7} & {14.1} \\
\rowcolor{cyan!50}
\modelnameproplus & O365, OI, V3D & RPN & 35 & \textbf{14.2} & \textbf{16.0} & \textbf{15.3} \\
\hline
GLIP-T (A) & O365 & GLIP-T(B) & 232 & 6.0 & 9.4  & 12.3 \\
GLIP-T (B) & O365 & GLIP-T(B) & 232 & 4.2 & 13.6  & 11.3 \\
GLIP-T (C) & O365, GoldG & GLIP-T(B) & 232 & 7.5 & 15.7  & 16.5 \\
GLIP-T & O365,GoldG,Cap4M & GLIP-T & 232 & 10.1 & 25.5  & 17.2 \\
GLIP-L & FourODs,GoldG,Cap24M & GLIP-L & 289 & 17.1 & 35.4 &  26.9 \\
\rowcolor{cyan!50}
\modelnamepro & O365 & GLIP-T(B) & 35 & 12.7 & 15.7 & 14.1 \\
\rowcolor{cyan!50}
\modelnamelite & O365, OI, V3D & GLIP-T & 22 & 20.0 & 24.2 &  21.1 \\
\rowcolor{cyan!50}
\modelnamepro & O365, OI, V3D & GLIP-T & 35 & 24.9 & 25.5 & 23.7 \\
\rowcolor{cyan!50}
\modelnameproplus & O365, OI, V3D & GLIP-T & 35 & 27.7 & 27.6 & 25.9 \\
\rowcolor{cyan!50}
\modelnameproplus & O365, OI, V3D & GLIP-L & 35 & \textbf{30.2} & \textbf{30.0} & \textbf{29.8} \\
\hline
\end{tabular}
\label{tab:main}
\end{table}



==> table/model_variants.tex <==
\begin{table}[]
	\centering
	    \begin{center}
% 		\makeatletter\def\@captype{table}\makeatother
        \begin{tabular}{l | c | c | c}
        Model &  SAM   & CLIP & Training data \\
        \hline
        \modelname{}-\texttt{BL(A)} & ViT-B & ViT-L & O365 \\
        \modelname{}-\texttt{BB} & ViT-B & ViT-B & O365, OI, V3D \\
        \modelname{}-\texttt{BL} & ViT-B & ViT-L & O365, OI, V3D \\
        \modelname{}-\texttt{HL} & ViT-H & ViT-L & O365, OI, V3D \\
       \hline
        \end{tabular}
		\caption{Details of \modelname{} variants.} 
		\label{tab:model_variants}
		\end{center}
\end{table}

==> table/panoptic_seg.tex <==
\begin{table}[tb]\centering
    \caption{Open-vocabulary panoptic segmentation performance}
    \label{tab:panoptic_seg}
    \resizebox{0.9\textwidth}{!}{
    \large
    \begin{tabular}{c|ccc|ccc|ccccc|cccc}
        \toprule
        & \multicolumn{3}{c|}{ADE20K} & \multicolumn{3}{c|}{COCO}  & \multicolumn{5}{c|}{Cityscapes} & \multicolumn{4}{c}{Mapillary Vistas}\\
       Method & PQ & AP & mIoU & PQ & AP & mIoU & PQ & SQ & RQ & AP & mIoU & PQ & SQ & RQ & mIoU \\
        \midrule
        A &  &   & 2& 3 & 4 & 5 &&&&&&&&& \\
        FC-CLIP & 26.8 & 16.8 & 34.1 & 54.4 & 44.6 & 63.7 & 44.0 &75.4 &53.6& 26.8 &56.2 &18.2 &57.7 &22.9 &27.9\\
        Ours &  & 2 & 3 & 4 & 6 & 5 &&&&&&&& \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> table/sam_clip.tex <==
\begin{table}[h]
\centering
\caption{The effective of  RegionSpot}
{
    {
    \begin{center}
    \begin{tabular}{l| c | c }
    method  & Proposals & AP$_{r}$  \\
    \shline
    SAM-CLIP  & SAM & 8.6 \\
    SAM-CLIP w/projector & SAM &9.6 \\
    \modelnamelite & SAM & 10.6 \\
    \hline\end{tabular}
    \end{center}
    }
    \label{tab:pipline}
}
\end{table}

==> table/semantic_seg.tex <==
\begin{table}[tb]\centering
    \caption{Open-vocabulary semantic segmentation performance}
    \label{tab:semantic_seg}
    \resizebox{0.9\textwidth}{!}{
    \large
    \begin{tabular}{c|c|cccccc}
        \toprule
        & & \multicolumn{6}{c}{mIoU}\\
       Method & Training Dataset & A-847 & PC-59 & A-150 & PC-59 & PAS-21 & PAS-20 \\
        \midrule
        FC-CLIP & COCO Panoptic & 14.8 &18.2& 34.1& 58.4& 81.8& 95.4\\
        Ours & COCO Panoptic & 2 & 3 & 4 & 6 & 5 & \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> table/train_ablation.tex <==
\begin{table}[ht]
	\centering
	\begin{center}
        \begin{tabular}{l | c | c | c | c}
       Prompt & AP$_{r}$ & AP$_{c}$ & AP$_{f}$ & AP  \\
        \shline
        baseline &  19.6 & 15.1 & 21.2 & 18.5 \\
        w/ mutiple boxes prompt &  23.2 & 19.2 & 25.0 & 22.1  \\
        w/ text prompt &  \textbf{24.9} & \textbf{21.6} & \textbf{25.5} & \textbf{23.7}   \\
        \hline\end{tabular}
	\caption{Ablation study on prompt engineering.} 
		\label{tab:trick}
  \vspace{-10pt}
		\end{center}
\end{table}
